Towards Latent Masked Image Modeling for Self-Supervised Visual Representation Learning

Masked Image Modeling (MIM) has emerged as a promising method for deriving visual representations from unlabeled image data by predicting missing pixels from masked portions of images. It excels in region-aware learning and provides strong initializations for various tasks, but struggles to capture high-level semantics without further supervised fine-tuning, likely due to the low-level nature of its pixel reconstruction objective. A promising yet unrealized framework is learning representations through masked reconstruction in latent space, combining the locality of MIM with the high-level targets. However, this approach poses significant training challenges as the reconstruction targets are learned in conjunction with the model, potentially leading to trivial or suboptimal solutions.Our study is among the first to thoroughly analyze and address the challenges of such framework, which we refer to as Latent MIM. Through a series of carefully designed experiments and extensive analysis, we identify the source of these challenges, including representation collapsing for joint online/target optimization, learning objectives, the high region correlation in latent space and decoding conditioning. By sequentially addressing these issues, we demonstrate that Latent MIM can indeed learn high-level representations while retaining the benefits of MIM models.

==> latex/20-related-work.tex <==
\section{Related Work}\label{sec:related-work}

%\pedro{Needs rewriting. All contents copied!}
%\pedro{@yibing: shorthen this 1 paragraph. dive directly into SSL for vision. we can simply merge 1st and 3rd paragraph.}

%SSL has a long history in machine learning~\cite{becker1992self,bromley1993signature,de1994learning,NIPS2004_42fe8808,chopra2005learning}.
%Motivated by the initial over-dependence of researchers and practitioners on high-quality labeled data, self-supervised learning seeks to build intelligent systems by training models to predict the structure of the data itself without the need for human supervision.

%Recent developments in SSL have delivered noteworthy successes in numerous areas of machine learning. For example, large language models trained to predict the next (or masked) words have been shown effective at few-shot inference~\cite{brown2020language}, paraphrasing~\cite{devlin2018bert}, question answering~\cite{devlin2018bert}, code completion~\cite{chen2021evaluating}, and show outstanding conversational skills~\cite{chatGPT}. 
%SSL in the form of contrastive predictive coding~\cite{cpc, schneider2019wav2vec, baevski2020wav2vec} has transformed speech processing applications, including speech recognition and sentiment analysis. 
%In computer vision, SSL has also captured the attention of the community for several years~\cite{hadsell2006dimensionality,ranzato2007unsupervised,mobahi2009deep,masci2011stacked,salakhutdinov2009deep,de1994learning,le2013building}.

%A wide range of self-supervised visual representation learning approaches have been investigated previously, including generative models such as denoising auto-encoders~\cite{vincent2008extracting}, sparse coding \cite{lee2007efficient,olshausen1996emergence,olshausen2000sparse}, masked image modeling~\cite{bao2021beit, he2022masked,feichtenhofer2022masked,assran2022masked}, inpainting~\cite{inpainting} and colorization~\cite{colorization,larsson2016learning,deshpande2015learning}, to methods that learn representations predictive of visual structure~\cite{context_pred,jigsaw,rotation}, or through invariance to visual transformations such as cropping or color jittering~\cite{exemplar,wu2018unsupervised,simclr, pirl,moco,swav,byol,mocov3,zbontar_barlowtwins,dino}.
%The two SSL frameworks that have shown the most promise in recent years are contrastive learning and masked image modeling.

% \paragraph{Self-Supervised Learning} aims to train models to understand data structure without human supervision. Its ability to learn highly informative visual representations from abundant unlabeled visual data has attracted considerable attention from the computer vision research community for several years~\cite{hadsell2006dimensionality,ranzato2007unsupervised,mobahi2009deep,masci2011stacked,salakhutdinov2009deep,de1994learning,le2013building}. A wide range of self-supervised visual representation learning approaches have been explored, including generative models such as denoising auto-encoders~\cite{vincent2008extracting}, sparse coding \cite{lee2007efficient,olshausen1996emergence,olshausen2000sparse}, masked image modeling~\cite{bao2021beit, he2022masked,feichtenhofer2022masked,assran2022masked}, inpainting~\cite{inpainting} and colorization~\cite{colorization,larsson2016learning,deshpande2015learning}, to methods that learn representations predictive of visual structure~\cite{context_pred,jigsaw,rotation}, or through invariance to visual transformations such as cropping or color jittering~\cite{exemplar,wu2018unsupervised,simclr, pirl,moco,swav,byol,mocov3,zbontar_barlowtwins,dino}.




==> latex/s-errata.tex <==
\section{Errata}

Table 7 in the main paper was inadvertently hidden due to a page transition. Please refer to the table provided below. This table will be incorporated into the main paper in the next revision.

\begin{table}[h!]
    
    \caption{\label{tab:in1k-cls}\textbf{Comparison with prior work on ImageNet-1k}.}
    \centering
    \resizebox{0.5\linewidth}{!}{\incls}
\end{table}

